Towards Multi-Agent Communication-Based Language Learning

We propose an interactive multimodal framework for language learning. Instead of being passively exposed to large amounts of natural text, our learners (implemented as feed-forward neural networks) engage in cooperative referential games starting from a tabula rasa setup, and thus develop their own language from the need to communicate in order to succeed at the game. Preliminary experiments provide promising results, but also suggest that it is important to ensure that agents trained in this way do not develop an adhoc communication code only effective for the game they are playing

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


\emph{Why learning through  communication is important?} From a theoretical
perspective, the primarily goal of language is for communicating our ideas and
beliefs. Moreover, communication through language is a collaborative process
between the discussants, i.e., although it might seem surprising, it makes
little sense to use language in such a way that people do not undertstand us!
Researchers refer to this use of language as ``pragmatic use'' and
computational models of \textbf{what} adopt this view by designing speakers
that accomodate for the the beliefs and understanding of the listerns (REFS).

From an empirical point of view, communication based-learning seems a viable
alternative of \emph{supervised learning}, a learning paradigm that requires
annotation of data, a general time-consuming, elaborating and expensive process
(depending on the task).  Perhaps the major drawback of supervised learning for
learning models of language use, is the fact that they assume a static
environment. Consider for example the case of referring expression generation
(REG), in which models are trained to produce referring expressions (RE) of
some referent given data of the form $\langle referent, context, RE^1,
RE^2\rangle$.  However, learning to generate RE in such a way completely
ignores the essense of the task itself, i.e., to produce an expression that a
listener would interpret in the desired way.  REG is just one example of tasks
where it would make sense that supervision would primarily come from the
success of the interaction. Unlike the static, fully supervised setup, speakers
have to take into consideration the dynamics of the environment, e.g., the
knowledge of current-state-of-affairs by the listener.


\emph{How can we design the communication-based learning environment?}
We could imagine of posible ways in which an agent could learn via interaction.
Probably, the most intuitive way is the one that involves directly the
\emph{human-in-the-loop}. The human user interacts with with the  agent in an
online manner and the agent learns a desired  model $\theta$ from the feedback
of the user. Probably one of the seminal attempts to learn in such a way was
the SHRLDU block-world program of Terry Winograd (REFS).  However, the obvious
limitations of this approach is the scaling up factor; having humans
interacting in an online manner with the agents makes development, learning and
testing very slow. Especially, in light of the fact that the majority of
current machine learning designs data-hungry models which need big amounts of
data, the cost of such an effort would simply be inconcievable!

Another possibility pertains to creating \emph{canned interactions}, i.e.,
scripted environments in the form of wizard-of-oz (REFS: Roadmap and Dialogue).
Such environments for communication similate a human user in the form of
pre-defined behaviour.  While this approachs fairs better with regards to
scalability, it requires a lot engineering effort in designing the right
behaviour of the environment.  An almost perfect balance between wizard-of-oz
environments and human-in-the-loop are the artificial environments (REFS:
Atari) in which agents learn via interacting with the environment. Still, up to
today, there are no such environments for learning language.

In this work, we propose to learn an agent via modeling communication and
interaction with another agent. Such multi-agent environments learn to perform
a task in such a way that communication between the two agents is maximized.












==> sections/marcos-temp-notes.tex <==
\section{Temp}

\paragraph{Intro} Very short: We outline a program for
multi-agent communication-based language learning. First, we motivate
our plans. We then present a pilot simulation, briefly discuss related
work, and we conclude with the lessons learned from this simulation.

\paragraph{Multi-agent referential games for language learning} This
should be quite a long section--as it is where you present the
``position'' of the position paper. 

The machine-learning approach to
language has been based on a static, passive, often supervised
approach: you get lots of annotated data, and you discover
patterns. Great to learn general statistical associations, but bad
for interactive communication, which is the core of what language is
about.

For this reason, interest in communication-based learning
environments: human-in-the-loop, scripted environments, multi-agent
setup!

Specifically, we consider the most basic act of communication,
with a \emph{referential game} (this is a term I've found in the
Galantucci et al's paper, apparently it is standard).

How do we ensure that the agents will not drift onto their own
language? We combine dynamic interactive learning with static
statistical learning of patterns from association.


\paragraph{A pilot simularion}

\paragraph{Related work}

\paragraph{Conclusion}


==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Communication-based learning}
Roadmap, AlphaGo, Winograd, people that use humans (will ask Yonatan), and perhaps Dialogue-based by Weston.

\paragraph{Refential games}
galantucci, some bayesiaon people and helbert Clark about conceptual packs when played with humans

\paragraph{Multi-agent Language Learning} 
Luc steels and naming experiment

